When does vapor pressure deficit drive or reduce evapotranspiration?

Increasing vapor pressure deficit (VPD) increases atmospheric demand for water. While increased evapotranspiration (ET) in response to increased atmospheric demand seems intuitive, plants are capable of reducing ET in response to increased VPD by closing their stomata. We examine which effect dominates the response to increasing VPD: atmospheric demand and increases in ET, or plant response (stomata closure) and decreases in ET. We use Penman-Monteith, combined with semi-empirical optimal stomatal regulation theory and underlying water use efficiency, to develop a theoretical framework for assessing ET response to VPD. The theory suggests that depending on the environment and plant characteristics, ET response to increasing VPD can vary from strongly decreasing to increasing, highlighting the diversity of plant water regulation strategies. The ET response varies due to: 1) climate, with tropical and temperate climates more likely to exhibit a positive ET response to increasing VPD than boreal and arctic climates; 2) photosynthesis strategy, with C3 plants more likely to exhibit a positive ET response than C4 plants; and 3) plant type, with crops more likely to exhibit a positive ET response, and shrubs and gymniosperm trees more likely to exhibit a negative ET response. These results, derived from previous literature connecting plant parameters to plant and climate characteristics, highlight the utility of our simplified framework for understanding complex land atmosphere systems in terms of idealized scenarios in which ET responds to VPD only. This response is otherwise challenging to assess in an environment where many processes co-evolve together.

==> param_fixed.tex <==
P & Pa & 100000.00 \\ 
$\gamma$ & Pa K$^{-1}$ & 64.50 \\ 
R$_{air}$ & J  K$^{-1}$ kg$^{-1}$ & 288.00 \\ 
c$_a$ & $\mu$ mol CO$_2$ mol$^{-1}$ air & 400.00 \\ 


==> param_varying.tex <==
g$_1$ & Pa$^{1/2}$ [kPa$^{1/2}$] & 63.25 [2.00] & 126.49 [4.00] & 189.74 [6.00] & Fig. 2, 7; \citeA{Medlyn_2017} \\ 
uWUE & $\mu$-mol C Pa$^{0.5}$ J$^{-1}$ ET [g C hPa$^{1/2}$ kg$^{-1}$ H$_2$O] & 2.33 [6.99] & 3.17 [9.52] & 4.01 [12.05] & Table 4; \citeA{Zhou_2015} \\ 
T & $^o$C & 10.00 & 20.00 & 30.00 & - \\ 
g$_a$ & m/s & 0.015 & 0.035 & 0.055 & - \\ 

